Underwater Image Restoration via Polymorphic Large Kernel CNNs

Underwater Image Restoration (UIR) remains a challenging task in computer vision due to the complex degradation of images in underwater environments. While recent approaches have leveraged various deep learning techniques, including Transformers and complex, parameter-heavy models to achieve significant improvements in restoration effects, we demonstrate that pure CNN architectures with lightweight parameters can achieve comparable results. In this paper, we introduce UIR-PolyKernel, a novel method for underwater image restoration that leverages Polymorphic Large Kernel CNNs. Our approach uniquely combines large kernel convolutions of diverse sizes and shapes to effectively capture long-range dependencies within underwater imagery. Additionally, we introduce a Hybrid Domain Attention module that integrates frequency and spatial domain attention mechanisms to enhance feature importance. By leveraging the frequency domain, we can capture hidden features that may not be perceptible to humans but are crucial for identifying patterns in both underwater and on-air images. This approach enhances the generalization and robustness of our UIR model. Extensive experiments on benchmark datasets demonstrate that UIR-PolyKernel achieves state-of-the-art performance in underwater image restoration tasks, both quantitatively and qualitatively. Our results show that well-designed pure CNN architectures can effectively compete with more complex models, offering a balance between performance and computational efficiency. This work provides new insights into the potential of CNN-based approaches for challenging image restoration tasks in underwater environments. The code is available at \href{https://github.com/CXH-Research/UIR-PolyKernel}{https://github.com/CXH-Research/UIR-PolyKernel}.

==> figtex/result_compare.tex <==
\begin{figure*}[ht]
%1
    \centering
    \begin{minipage}[b]{1\linewidth}
        \begin{minipage}[b]{.12\linewidth}
            \centering
            \includegraphics[width=\linewidth]{figs/euvp_test_p114_input.jpg}
        \end{minipage}
        \begin{minipage}[b]{.12\linewidth}
            \centering
            \includegraphics[width=\linewidth]{figs/euvp_test_p114_ADPCC.jpg}
        \end{minipage}
        \begin{minipage}[b]{.12\linewidth}
            \centering
            \includegraphics[width=\linewidth]{figs/euvp_test_p114_GUPDM.jpg}
        \end{minipage}
        \begin{minipage}[b]{.12\linewidth}
            \centering
            \includegraphics[width=\linewidth]{figs/euvp_test_p114_URSCT.jpg}
        \end{minipage}
        \begin{minipage}[b]{.12\linewidth}
            \centering
            \includegraphics[width=\linewidth]{figs/euvp_test_p114_Semi_UIR.jpg}
        \end{minipage}
        \begin{minipage}[b]{.12\linewidth}
            \centering
            \includegraphics[width=\linewidth]{figs/euvp_test_p114_WWPF.jpg}
        \end{minipage}
        \begin{minipage}[b]{.12\linewidth}
            \centering
            \includegraphics[width=\linewidth]{figs/euvp_test_p114_ours.jpg}
        \end{minipage}
        \begin{minipage}[b]{.12\linewidth}
            \centering
            \includegraphics[width=\linewidth]{figs/euvp_test_p114_target.jpg}
        \end{minipage}
    \end{minipage}

%2
    \begin{minipage}[b]{1\linewidth}
        \begin{minipage}[b]{.12\linewidth}
            \centering
            \includegraphics[width=\linewidth]{figs/euvp_test_p52_input.jpg}
        \end{minipage}
        \begin{minipage}[b]{.12\linewidth}
            \centering
            \includegraphics[width=\linewidth]{figs/euvp_test_p52_ADPCC.jpg}
        \end{minipage}
        \begin{minipage}[b]{.12\linewidth}
            \centering
            \includegraphics[width=\linewidth]{figs/euvp_test_p52_GUPDM.jpg}
        \end{minipage}
        \begin{minipage}[b]{.12\linewidth}
            \centering
            \includegraphics[width=\linewidth]{figs/euvp_test_p52_URSCT.jpg}
        \end{minipage}
        \begin{minipage}[b]{.12\linewidth}
            \centering
            \includegraphics[width=\linewidth]{figs/euvp_test_p52_semi_UIR.jpg}
        \end{minipage}
        \begin{minipage}[b]{.12\linewidth}
            \centering
            \includegraphics[width=\linewidth]{figs/euvp_test_p52_WWPF.jpg}
        \end{minipage}
        \begin{minipage}[b]{.12\linewidth}
            \centering
            \includegraphics[width=\linewidth]{figs/euvp_test_p52_ours.jpg}
        \end{minipage}
        \begin{minipage}[b]{.12\linewidth}
            \centering
            \includegraphics[width=\linewidth]{figs/euvp_test_p52_target.jpg}
        \end{minipage}
    \end{minipage}
%3
    \begin{minipage}[b]{1\linewidth}
        \begin{minipage}[b]{.12\linewidth}
            \centering
            \includegraphics[width=\linewidth]{figs/lsui_2211_input.jpg}
        \end{minipage}
        \begin{minipage}[b]{.12\linewidth}
            \centering
            \includegraphics[width=\linewidth]{figs/lsui_2211_ADPCC.jpg}
        \end{minipage}
        \begin{minipage}[b]{.12\linewidth}
            \centering
            \includegraphics[width=\linewidth]{figs/lsui_2211_GUPDM.jpg}
        \end{minipage}
        \begin{minipage}[b]{.12\linewidth}
            \centering
            \includegraphics[width=\linewidth]{figs/lsui_2211_URSCT.jpg}
        \end{minipage}
        \begin{minipage}[b]{.12\linewidth}
            \centering
            \includegraphics[width=\linewidth]{figs/lsui_2211_Semi_UIR.jpg}
        \end{minipage}
        \begin{minipage}[b]{.12\linewidth}
            \centering
            \includegraphics[width=\linewidth]{figs/lsui_2211_WWPF.jpg}
        \end{minipage}
        \begin{minipage}[b]{.12\linewidth}
            \centering
            \includegraphics[width=\linewidth]{figs/lsui_2211_ours.jpg}
        \end{minipage}
        \begin{minipage}[b]{.12\linewidth}
            \centering
            \includegraphics[width=\linewidth]{figs/lsui_2211_target.jpg}
        \end{minipage}
    \end{minipage}

%4
    \begin{minipage}[b]{1\linewidth}
        \begin{minipage}[b]{.12\linewidth}
            \centering
            \includegraphics[width=\linewidth]{figs/lsui_2338_input.jpg}
        \end{minipage}
        \begin{minipage}[b]{.12\linewidth}
            \centering
            \includegraphics[width=\linewidth]{figs/lsui_2338_ADPCC.jpg}
        \end{minipage}
        \begin{minipage}[b]{.12\linewidth}
            \centering
            \includegraphics[width=\linewidth]{figs/lsui_2338_GUPDM.jpg}
        \end{minipage}
        \begin{minipage}[b]{.12\linewidth}
            \centering
            \includegraphics[width=\linewidth]{figs/lsui_2338_URSCT.jpg}
        \end{minipage}
        \begin{minipage}[b]{.12\linewidth}
            \centering
            \includegraphics[width=\linewidth]{figs/lsui_2338_Semi_UIR.jpg}
        \end{minipage}
        \begin{minipage}[b]{.12\linewidth}
            \centering
            \includegraphics[width=\linewidth]{figs/lsui_2338_WWPF.jpg}
        \end{minipage}
        \begin{minipage}[b]{.12\linewidth}
            \centering
            \includegraphics[width=\linewidth]{figs/lsui_2338_ours.jpg}
        \end{minipage}
        \begin{minipage}[b]{.12\linewidth}
            \centering
            \includegraphics[width=\linewidth]{figs/lsui_2338_target.jpg}
        \end{minipage}
    \end{minipage}

%5
    \begin{minipage}[b]{1\linewidth}
        \begin{minipage}[b]{.12\linewidth}
            \centering
            \includegraphics[width=\linewidth]{figs/uieb_614_img_input.png}
        \end{minipage}
        \begin{minipage}[b]{.12\linewidth}
            \centering
            \includegraphics[width=\linewidth]{figs/uieb_614_img__ADPCC.png}
        \end{minipage}
        \begin{minipage}[b]{.12\linewidth}
            \centering
            \includegraphics[width=\linewidth]{figs/uieb_614_img_GUPDM.png}
        \end{minipage}
        \begin{minipage}[b]{.12\linewidth}
            \centering
            \includegraphics[width=\linewidth]{figs/uieb_614_img_URSCT.png}
        \end{minipage}
        \begin{minipage}[b]{.12\linewidth}
            \centering
            \includegraphics[width=\linewidth]{figs/uieb_614_img_Semi_UIR.png}
        \end{minipage}
        \begin{minipage}[b]{.12\linewidth}
            \centering
            \includegraphics[width=\linewidth]{figs/uieb_614_img_WWPF.png}
        \end{minipage}
        \begin{minipage}[b]{.12\linewidth}
            \centering
            \includegraphics[width=\linewidth]{figs/uieb_614_img_ours.png}
        \end{minipage}
        \begin{minipage}[b]{.12\linewidth}
            \centering
            \includegraphics[width=\linewidth]{figs/uieb_614_img_target.png}
        \end{minipage}
    \end{minipage}

%6
    \begin{minipage}[b]{1\linewidth}
        \begin{minipage}[b]{.12\linewidth}
            \centering
            \centerline{\includegraphics[width=\linewidth]{figs/uieb_908_img_input.png}}
            \centerline{(a) Input}\medskip
        \end{minipage}
        \begin{minipage}[b]{.12\linewidth}
            \centering
            \centerline{\includegraphics[width=\linewidth]{figs/uieb_908_img_ADPCC.png}}
            \centerline{(b) ADPCC}\medskip
        \end{minipage}
        \begin{minipage}[b]{0.12\linewidth}
            \centering
            \centerline{\includegraphics[width=\linewidth]{figs/uieb_908_img_GUPDM.png}}
            \centerline{(c) GUPDM}\medskip
        \end{minipage}
        \begin{minipage}[b]{.12\linewidth}
            \centering
            \centerline{\includegraphics[width=\linewidth]{figs/uieb_908_img_URSCT.png}}
            \centerline{(d) URSCT}\medskip
        \end{minipage}
        \begin{minipage}[b]{.12\linewidth}
            \centering
            \centerline{\includegraphics[width=\linewidth]{figs/uieb_908_img_Semi_UIR.png}}
            \centerline{(e) Semi UIR}\medskip
        \end{minipage}
        \begin{minipage}[b]{.12\linewidth}
            \centering
            \centerline{\includegraphics[width=\linewidth]{figs/uieb_908_img_WWPF.png}}
            \centerline{(f) WWPF}\medskip
        \end{minipage}
        \begin{minipage}[b]{.12\linewidth}
            \centering
            \centerline{\includegraphics[width=\linewidth]{figs/uieb_908_img_ours.png}}
            \centerline{(g) Ours}\medskip
        \end{minipage}
        \begin{minipage}[b]{0.12\linewidth}
            \centering
            \centerline{\includegraphics[width=\linewidth]{figs/uieb_908_img_target.png}}
            \centerline{(h) Target}\medskip
        \end{minipage}
    \end{minipage}
    
    \caption{The qualitative results of comparing the methods on three different datasets: EUVP, LSUI and UIEB.} 
    \label{fig:comp}
\end{figure*}

==> related.tex <==
Traditional:
UNTV~\cite{xie2021variational} employs a variational framework with a red channel prior to effectively address underwater image degradation by incorporating forward scattering, achieving superior dehazing and deblurring compared to other methods.
MLLE~\cite{zhang2022underwater} employs a minimum color loss principle and adaptive contrast techniques to enhance underwater images, resulting in vivid colors and detailed clarity.
ROP~\cite{liu2022rank} introduces a rank-one prior framework for real-time scene recovery across various conditions, including underwater environments.
ADPCC~\cite{zhou2023underwater} integrates a comprehensive imaging model with channel intensity and adaptive dark pixel strategies, enhancing underwater image restoration by addressing uneven lighting and diverse conditions.
WWPF~\cite{zhang2023underwater} addresses underwater image degradation through a weighted wavelet visual perception fusion approach, combining global and local contrast enhancements to deliver superior image quality.


Learning based:
WaterNet \cite{li2019underwater} presents an underwater image enhancement network trained on a new benchmark, UIEB, comprising 950 real-world images. 
UColor \cite{li2021underwater} is a network designed to enhance underwater images by leveraging medium transmission-guided multi-color space embedding. It uses a multi-color space encoder and attention mechanism to integrate features, significantly improving image quality.
CLUIE-Net \cite{li2022beyond} is a comparative learning framework for underwater image enhancement, addressing the scarcity of enhancement references by learning from multiple candidates.
STSC \cite{wang2022semantic} employs an efficient semantic-aware model to enhance underwater images, refining features for improved quality and applicability in salient object detection.
SFGNet \cite{zhao2024toward} is a UIE framework leveraging spatial-frequency interaction and gradient maps. It features a dense spatial-frequency fusion network and a gradient-aware corrector to enhance image details and structures.
PUGAN \cite{cong2023pugan} combines GANs and physical models for underwater image enhancement, using a Parameters Estimation subnetwork for color correction and a Two-Stream Interaction Enhancement subnetwork to refine key areas.
TUDA \cite{wang2023domain} is a Two-phase Underwater Domain Adaptation network designed to address domain gaps in underwater image enhancement.
U-Transformer \cite{peng2023u} U-Transformer uses a U-shape Transformer with CMSFFT and SGFMT modules for underwater image enhancement, leveraging a large dataset and a novel multi-color space loss function to achieve high performance.
URSCT \cite{ren2022reinforced} is a U-Net-based method that incorporates a reinforced Swin-Convs Transformer for superresolution.
Semi-UIR \cite{huang2023contrastive} is a semi-supervised framework for underwater image restoration that utilizes a mean-teacher approach to leverage unlabeled data.
USUIR \cite{fu2022unsupervised} is an unsupervised method for restoring underwater images by leveraging homology between raw and re-degraded images, minimizing restoration error, and achieving high performance in speed and quality.
GUPDM \cite{mu2023generalized} enhances underwater images by simulating various scenes and using dynamic structures to adaptively extract information, with multi-scale feature extraction for different water types.
SyreaNet \cite{wen2023syreanet} employs a novel UIE framework that integrates synthetic and real data using a revised underwater image formation model and domain adaptation strategies.



==> tabletex/nonref.tex <==
\begin{table}[ht]
\centering
\caption{Quantitative comparison of deep learning methods on the unpaired test sets UIEB, EUVP, and RUIE without reference targets using the \textbf{UCIQE} metric.}
\label{tab:nonref}
\begin{tabular}{lcccc}
\toprule
Method        & UIEB  & EUVP  & RUIE  & Average \\ \midrule
UColor        & 0.352 & 0.322 & 0.256 & 0.310   \\
CLUIE-Net     & 0.394 & 0.349 & 0.331 & 0.358   \\
STSC          & 0.393 & 0.385 & 0.378 & 0.386   \\
TACL          & 0.421 & 0.432 & 0.419 & 0.424   \\
UIE-WD        & 0.403 & 0.380 & 0.343 & 0.375   \\
URSCT         & 0.414 & 0.398 & 0.384 & 0.399   \\
USUIR         & 0.431 & 0.422 & 0.390 & 0.414   \\
GUPDM         & 0.412 & 0.382 & 0.380 & 0.392   \\
PUGAN         & 0.414 & 0.412 & 0.369 & 0.399   \\
Semi-UIR      & 0.417 & 0.400 & 0.385 & 0.400   \\
SyreaNet      & 0.433 & 0.436 & 0.391 & 0.420   \\
TUDA          & 0.422 & 0.405 & 0.392 & 0.406   \\
U-Transformer & 0.424 & 0.406 & 0.409 & 0.413   \\
SFGNet        & 0.412 & 0.388 & 0.390 & 0.397   \\
Ours          & 0.437 & 0.415 & 0.440 & 0.431  \\ \bottomrule
\end{tabular}
\end{table}

==> unrelated.tex <==
HLRP~\cite{zhuang2022underwater} utilizes hyper-laplacian reflectance priors in a retinex model to enhance underwater images, effectively improving detail and color accuracy.

Other methods:
WCID~\cite{chiang2011underwater} is a systematic approach to underwater image enhancement, addressing light scattering and color change by integrating dehazing and wavelength compensation.
Fusion~\cite{ancuti2012enhancing} is a framework designed to enhance underwater images and videos by deriving inputs and weights from the degraded images themselves.
min\_info\_loss~\cite{li2016underwater} leverages a minimum information loss principle to improve visibility and color. It offers dehazing and contrast enhancement to produce images suitable for display and detailed analysis
IBLA~\cite{peng2017underwater} is a depth estimation method for underwater scenes using image blurriness and light absorption, overcoming limitations caused by varying lighting conditions.
Sea-thru~\cite{akkaynak2019sea} offers a robust method for recovering lost colors in underwater images by employing a physically accurate model instead of the atmospheric model. Utilizing RGBD images, it calculates backscatter and estimates spatially varying illuminants, enhancing underwater exploration capabilities.
H. Wang et al.~\cite{wang2023underwater} propose correcting underwater color disparities to align with natural consistencies, using adaptive compensation and contrast enhancement to improve image quality without deep learning. 
UJDM ~\cite{shen2024polarization} introduces a polarization-driven solution to enhance underwater images by addressing light scattering and uneven illumination. Utilizing polarization distinctions, it improves contrast and detail.

UWCNN \cite{li2020underwater} develops a convolutional neural network for enhancing underwater images using scene priors, bypassing parameter estimation.

Shallow-UWNet \cite{naik2021shallow} is a lightweight neural network designed for underwater image enhancement, it generalizes well across synthetic and real-world datasets, making it suitable for portable devices in underwater exploration.
PUIE-Net \cite{fu2022uncertainty} utilizes a probabilistic network that tackles underwater image enhancement by learning enhancement distributions instead of relying solely on reference maps.
DeepWaveNet \cite{sharma2023wavelength} addresses underwater image restoration by considering color channel traversal ranges and refining features through an attentive skip mechanism. 
$\mathrm{NU^2Net}$ \cite{guo2023underwater} is a simple U-shape UIE network composed of Conv-IN-ELU blocks, enhanced by a normalization tail to boost performance.
UGAN \cite{fabbri2018enhancing} leverages Generative Adversarial Networks to enhance underwater images, improving visual data quality for autonomous vehicles and boosting accuracy in tasks like diver tracking.
CWR \cite{han2021single} develops contrastive learning and generative adversarial networks within an unsupervised image-to-image translation framework for underwater image restoration.
TACL \cite{liu2022twin} introduces an object-guided twin adversarial contrastive learning method for underwater image enhancement, optimizing both visual appeal and task performance.
UIE-WD \cite{ma2022wavelet} employs a wavelet-based dual-stream network to tackle color cast and blurriness in underwater images.
CCMSRNet \cite{qi2023deep} advances underwater image processing by integrating Color Correction and Multi-scale Retinex techniques with Hybrid Convolution-Axial Attention Blocks.
URanker \cite{guo2023underwater}
DGD-cGAN \cite{gonzalez2024dgd} is an innovative approach for enhancing underwater images by addressing color cast and blur through a Dual Generator Dewatering cGAN.
HCLR-Net \cite{zhou2024hclr} leverages Hybrid Contrastive Learning Regularization to enhance underwater images, using innovative negative sample construction to bypass paired data needs. 
CECF~\cite{cong2024underwater} introduces a novel approach for underwater image enhancement by combining color enhancement with color fine-tuning capabilities, allowing diverse color outcomes.
